On Using Monolingual Corpora in Neural Machine Translation

Recent work on end-to-end neural network-based architectures for machine translation has shown promising results for En-Fr and En-De translation. Arguably, one of the major factors behind this success has been the availability of high quality parallel corpora. In this work, we investigate how to leverage abundant monolingual corpora for neural machine translation. Compared to a phrase-based and hierarchical baseline, we obtain up to $1.96$ BLEU improvement on the low-resource language pair Turkish-English, and $1.59$ BLEU on the focused domain task of Chinese-English chat messages. While our method was initially targeted toward such tasks with less parallel data, we show that it also extends to high resource languages such as Cs-En and De-En where we obtain an improvement of $0.39$ and $0.47$ BLEU scores over the neural machine translation baselines, respectively.

==> abstract.tex <==
    Recent works on using end-to-end RNN based architectures for machine translation have shown
    success for English and French. In this paper, we investigate the effect of integrating an external 
    language model for neural machine translation for low resource languages such as Chinese and Turkish. 
    We did our experiments on IWSLT 2014 and Openmt 2015 datasets. We proposed two different methods of
    integrating language models into the neural machine translation system. We were
    able to obtain improvements compared to several baselines including moses with CSLM integration 
    and Neural Machine Translation systems without any language model integration.


